I Know What You Meme, Even If it Emerged Today: Understanding Evolving Memes through Open-World Knowledge Acquisition

Multimodal memes are dynamic and often require up to date background knowledge for interpretation. Existing methods often overlook such knowledge or rely on fixed parametric knowledge of pretrained models that may be incomplete, outdated, or unavailable for emerging memes. We introduce Query Retrieve Conclude, a zero shot framework that identifies missing knowledge, retrieves open web evidence, and synthesizes evidence grounded background knowledge for meme understanding and detection. We also introduce a curated meme understanding benchmark of recent memes from 2024 to 2026 with external background knowledge annotations. Experiments on three meme understanding datasets and five meme detection tasks show that our framework improves knowledge recovery, meme understanding and downstream detection over zero shot baselines.

==> sections/04_design.tex <==
\section{Evaluation of Informational Bias}

==> sections/prev_intro.tex <==

%abstract
Existing supervised models to zero-shot learning with Large Vision-Language Models (LVLMs) often either overlook the background knowledge needed for interpretation or rely on fixed parametric knowledge that may be incomplete, outdated, or unavailable for newly emerging memes. 
We introduce \textit{Query-Retrieve-Conclude}, a three-stage framework for automated meme understanding under dynamic open-world contexts.
Instead of directly prompting a model to explain or classify a meme, our framework explicitly maps visual-textual friction into an actionable knowledge gap via search-oriented question generation (\textit{Query}), fetches real-time external evidence to construct grounded answers (\textit{Retrieve}), and consolidates these fragments into unified background knowledge statements for downstream tasks (\textit{Conclude}).
To evaluate our framework against strict temporal distribution shifts, we introduce KYM, a highly curated evaluation dataset capturing volatile internet phenomena from 2024 to 2026.
Experiments on three meme understanding datasets including our KYM and five meme detection tasks show that our evidence-grounded framework improves both background knowledge recovery and social abuse related meme detection over zero-shot background knowledge generation.

\section{Introduction}
%\crcomment{Your previous version was in prev_intro.tex} 

\begin{figure}[t!]
    \centering
    \includegraphics[
        width=0.95\linewidth,
        trim={0cm 0cm 0cm 0cm},
        clip
    ]{latex/pic/intro.png}
    \caption{
    An example illustrating the open-world knowledge gap in meme understanding. 
The meme \protect\footnotemark{} requires background knowledge beyond its visible image and text, including Confucius-related wordplay, and the Strait of Hormuz contex. 
Direct zero-shot prompting misses this context, while our Query-Retrieve-Conclude framework recovers evidence-grounded background knowledge to support the correct downstream prediction.
    }
    % \caption[Overview of automated meme understanding and detection.]{
    % Given an input meme\protect\footnotemark{} and its embedded text, our goal is to support automated meme understanding and detection. Compared with zero-shot prompting (\textcolor{pink}{in pink}), our pipeline recovers reference-aligned background knowledge and uses it as contextual evidence to support more accurate downstream prediction (\textcolor{green!60!black}{in green}).
    % }
    \label{fig:intro}
\end{figure}
\footnotetext{Source of the meme used in this figure: \url{https://knowyourmeme.com/}.}

Internet memes are inherently dynamic and temporally evolving forms of online communication.\footnote{\url{https://en.wikipedia.org/wiki/Memetics}} Their meanings often depend on recent news, viral templates, emerging public controversies, cultural references, or newly formed associations between public figures and events \cite{valensise2021entropy}. Yet, these contextual elements are often absent from the meme image and text themselves. Even with the rapid advancement of LVLMs, the relevant background knowledge may still be incomplete, outdated, or unavailable in a model's parametric memory depending on its knowledge cutoff time.\footnote{\url{https://en.wikipedia.org/wiki/Knowledge_cutoff}} This makes background knowledge acquisition a challenging yet important problem for meme understanding.

For example, the meme in Figure~\ref{fig:intro} requires recognizing the two depicted figures Donald Trump and Confucius, while also interpreting the embedded textual wordplay. Specifically, the phrase ``CON-FUSE-US'' simultaneously evokes ``Confuciu''  and the English word``confus'', creating a layered pun that relies on both linguistic and cultural background knowledge.\footnote{Fun Fact or Additional background knowledge: The Mandarin Chinese pronunciation of Kǒngfūzǐ \zh{(孔夫子)} can be perceived as phonetically similar to ``confuse'' in English.}
Beyond this wordplay, understanding this meme also requires historical background knowledge that Iran blocked the shipping traffic through the Strait of Hormuz since 28 February 2026 and that the United States imposed a naval blockade on Iran following the failure of the Islamabad Talks to end the 2026 Iran war.\footnote{\url{https://en.wikipedia.org/wiki/2026_Strait_of_Hormuz_crisis}; \url{https://en.wikipedia.org/wiki/2026_United_States_naval_blockade_of_Iran}}
As a result, the knowledge required to interpret a meme may be absent from the meme image and text themselves, outdated, or unreliable in the parametric memory of a pretrained vision-language model (VLM). This creates an open-world knowledge gap for automated meme understanding: the model must not only perceive the meme, but also acquire the missing background knowledge needed for interpretation.

% Prior work has explored fusion-based multimodal architectures, prompting and in-context learning with large VLMs, and knowledge-enhanced methods for meme understanding ~\cite{lee2021disentangling,pramanick2021momenta,cao2022prompting,cao2023pro,lin2024goat,hee2025demystifying,chen2025adammeme,lin2025explainhm++}. 
Recent work has begun to examine the role of background knowledge in meme understanding. For example,  MemeIntent~\cite{park2024memeintent}, MemeQA~\cite{nguyen2025memeqa}, and MemeInterpret~\cite{park2025memeinterpret}, introduce human-annotated intents, rationales, or background knowledge for evaluating meme understanding. Other methods, such as CROSS-ALIGN+~\cite{tripathi2026they}, incorporate existing cultural resources, while MemeAgent~\cite{lin2025ask} uses agent-style question-answering discussions for social abuse detection. Despite these advances, these approaches often rely on task-specific training data, human-annotated background knowledge, predefined cultural resources, or the model's implicit parametric knowledge. 

\textbf{Our Approach}. 
To address this limitation, we propose a Query-Retrieve-Conclude framework for automated meme understanding.
Rather than directly asking a VLM to explain or classify a meme, our framework decomposes meme interpretation into an explicit evidence-seeking process. 
The \textbf{Query} stage identifies missing knowledge by using reverse image search, caption generation, and question generation to produce search-oriented questions. 
The \textbf{Retrieval} stage retrieves external textual evidence for each question and generates evidence-grounded answers. 
The \textbf{Conclude} stage synthesizes the resulting question-answer pairs into explicit background knowledge statements, following evidence-statement formulations in recent retrieval evaluation work~\cite{cao2025averimatec,akhtar2026ev2r}, and uses these statements as contextual evidence for downstream task. 
This differs from direct zero-shot background knowledge generation, where a model is asked to infer the missing context in one step. 
Such direct generation can produce plausible but unsupported knowledge, especially when the meme refers to recent or evolving events. 
Our framework instead makes the missing-knowledge discovery process explicit: it first generates search-oriented questions, retrieves evidence for those questions, and only then synthesizes background knowledge statements for detection.
To the best of our knowledge, we are the first to explicitly address meme understanding and detection under dynamic and evolving meme contexts as a query-driven, retrieval-grounded, and conclusion-oriented knowledge acquisition problem. 
In summary, our contributions are as follows:
\begin{itemize}
    \item We propose the first framework that tackles dynamic and evolving meme contexts for meme understanding.
    
    \item We design a three-stage framework that recovers interpretable meme-specific background knowledge without task-specific fine-tuning.

    \item We curate \textbf{KYM}, a dataset of recent memes involving events from 2024-2026 with annotated external background knowledge, and conduct experiments on three meme understanding datasets and five meme detection tasks, demonstrating that our evidence-grounded knowledge improves zero-shot meme detection over direct prompting and zero-shot background knowledge generation.
\end{itemize}

% A meme is not simply an image, a caption, or a set of external facts in isolation; rather, its meaning emerges from the interaction among visual cues, textual cues, and culturally situated background knowledge~\cite{cao2022prompting,cao2023pro,park2024memeintent,nguyen2025memeqa}.
% As \cite{nguyen2025memeqa} observed, "Automated meme understanding requires systems to demonstrate fine-grained visual recognition, commonsense reasoning, and extensive
% cultural knowledge." \footnote{We position our proposed automated meme understanding and detection framework as complementary to the dimensions of holistic meme understanding discussed in~\cite{nguyen2025memeqa}.} 
